Agon: A Scalable Competitive Scheduler for Large Heterogeneous Systems

This work proposes a competitive scheduling approach, designed to scale to large heterogeneous multicore systems. This scheduler overcomes the challenges of (1) the high computation overhead of near-optimal schedulers, and (2) the error introduced by inaccurate performance predictions. This paper presents Agon, a neural network-based classifier that selects from a range of schedulers, from simple to very accurate, and learns which scheduler provides the right balance of accuracy and overhead for each scheduling interval. Agon also employs a de-noising frontend allowing the individual schedulers to be tolerant towards noise in performance predictions, producing better overall schedules. By avoiding expensive scheduling overheads, Agon improves average system performance by 6\% on average, approaching the performance of an oracular scheduler (99.1% of oracle performance).

==> images/slopes.tex <==
\begin{figure*}[t]
\centering
    \subfloat[][Scheduling approach has low impact]{ 
        \includegraphics[height=5cm, keepaspectratio]{images/graphs/slope_1.pdf}
    }
    \quad
    \subfloat[][Prediction error impacts hungarian algorithm significantly]{ 
        \includegraphics[height=5cm, keepaspectratio] {images/graphs/slope_2.pdf}
    }\\
    \subfloat[][High number of bad schedules makes smart random a good choice]{ 
        \includegraphics[height=5cm, keepaspectratio]{images/graphs/slope_3.pdf}
    }
    \quad
    \subfloat[][Impossible problem instance (all schedules are bad)]{ 
        \includegraphics[height=5cm, keepaspectratio]{images/graphs/slope_4.pdf}
    }
\caption{Four handpicked examples of problem instances and their schedule slope.}
\label{fig:slopes}
\end{figure*}

==> tables/deep_classifier.tex <==
\begin{table}
\begin{center}

\begin{tabular}{|cccc|}
\hline
\textbf{Layer ID} & \textbf{Layer Type} & \textbf{\# Nodes} & \textbf{Activation} \\ \hline
1 & Dense & 128 & ReLU \\ 
2 & Dense & 32 & ReLU \\ 
3 & Dense & 6 & softmax \\ \hline
\end{tabular}

\end{center}
\caption{Layer breakdown: Deep FFN classifier}
\label{tab:deep_classifier}
\end{table}

==> tables/simple_denoiser.tex <==
\begin{table}[]
\begin{center}

\begin{tabular}{|cccc|}
\hline
\textbf{Layer ID} & \textbf{Layer Type} & \textbf{\# Nodes} & \textbf{Activation} \\ \hline
1 & Dense & 32 & ReLU \\ 
2 & Dense & 64 & ReLU \\ \hline
\end{tabular}

\end{center}
\caption{Layer breakdown: Simple FFN denoiser}
\label{tab:simple_denoiser}
\end{table}
